Mechanics, readout and cooling systems of the Mu3e experiment

Mu3e is an upcoming experiment at Paul Scherrer Institut in the search for the strongly suppressed decay of $\mu\rightarrow eee$. It will use an ultra-lightweight silicon pixel detector using thinned HV-CMOS MAPS chips. Multiple Coulomb scattering is further kept under control with using high density interconnects made of aluminium and operating the detector in a helium atmosphere. More than 1 m2 of instrumented surface will produce about 3.3 kW of heat ($\leq$ 250 mW/cm2). Traditional cooling approaches are in conflict with the low-mass requirements, hence a gaseous helium flow cooling system will be implemented. This talk will give a report on the successful data transmission tests with the aluminium interconnects at target speeds of 1.25 Gbit/s under realistic condition. The final proof-of-concept of the helium cooling has been achieved with comprehensive cooling simulations and successfully confirmed with laboratory measurements using a full-scale mock-up of the vertex pixel detector.

==> graphics/cooling/L34_temps.tex <==
\pgfplotstableread[col sep = semicolon]{./graphics/cooling/L34-ABC-temps.csv}\loadedtable

\begin{tikzpicture}
\begin{groupplot}[
group style={group size= 1 by 3, vertical sep=0.7cm},
linien,
legend cell align= {left},
legend style ={at={(1,1)},anchor=north east},
width=0.9\linewidth,
scale only axis,
xmin = -580,
xmax = 580,
ymin=0,
xtick distance = 100,
enlarge x limits =0,
unbounded coords=jump,
legend columns = 6,
legend style={at={(0.5,1)},anchor= south},
title style={at={(xticklabel cs:0.5,23)},text width=0.9\linewidth}
]

\nextgroupplot[ylabel={Temp. $\unik{^\circ C}$}, title = MuPix chip temperature, height=2cm, xtick=\empty]
\addlegendimage{empty legend} 
\addplot+[emphasizeopa=-580:-210 with orange and 0.1, emphasizeopa=-180:180 with blue and 0.1, emphasizeopa=210:580 with green and 0.1,] table [x=Z, y=S4-maxT, col sep=semicolon] {\loadedtable};
\addplot table [x=Z, y=S3-maxT, col sep=semicolon] {\loadedtable};
\addlegendimage{empty legend} 
\addplot table [x=Z, y=S4-T, col sep=semicolon] {\loadedtable};
\addplot table [x=Z, y=S3-T, col sep=semicolon] {\loadedtable};
\legend{\textbf{max:}, L4, L3, \textbf{mean:}, L4, L3}

\nextgroupplot[xlabel={Distance from midplane $z \unik{mm}$}, ylabel={Temp. $\unik{^\circ C}$}, title = Global helium temperature, height=2cm]
\addplot table [x=Z, y=Global-maxT, col sep=semicolon] {\loadedtable};
\addplot+[line width=1pt] table [x=Z, y=Global-T, col sep=semicolon] {\loadedtable};
\legend{max $T$, mean $T$,}
\end{groupplot}

\end{tikzpicture}
